Multilevel CNNs for Parametric PDEs based on Adaptive Finite Elements

A neural network architecture is presented that exploits the multilevel properties of high-dimensional parameter-dependent partial differential equations, enabling an efficient approximation of parameter-to-solution maps, rivaling best-in-class methods such as low-rank tensor regression in terms of accuracy and complexity. The neural network is trained with data on adaptively refined finite element meshes, thus reducing data complexity significantly. Error control is achieved by using a reliable finite element a posteriori error estimator, which is also provided as input to the neural network. The proposed U-Net architecture with CNN layers mimics a classical finite element multigrid algorithm. It can be shown that the CNN efficiently approximates all operations required by the solver, including the evaluation of the residual-based error estimator. In the CNN, a culling mask set-up according to the local corrections due to refinement on each mesh level reduces the overall complexity, allowing the network optimization with localized fine-scale finite element data. A complete convergence and complexity analysis is carried out for the adaptive multilevel scheme, which differs in several aspects from previous non-adaptive multilevel CNN. Moreover, numerical experiments with common benchmark problems from Uncertainty Quantification illustrate the practical performance of the architecture.

==> macros.tex <==


\newtheorem{theorem}{Theorem}[section]
\newtheorem{definition}[theorem]{Definition}
\newtheorem{lemma}[theorem]{Lemma}%[section]
\newtheorem{remark}[theorem]{Remark}%[section]

% MATH -------------------------------------------------------------------------------------------

%\newcommand{\abs}[1]{\left| #1 \right|}
%\newcommand{\norm}[1]{\left\lVert #1 \right\rVert}
\newcommand{\scpr}[1]{\left\langle #1 \right\rangle}
\newcommand{\bb}[1]{\mathbb{#1}}
%\newcommand{\argmax}{\text{argmax}}
\newcommand{\spa}{\text{span}}
\newcommand{\anorm}[1]{\left|\lVert #1 \rVert \right|}
\newcommand{\xmark}{\ding{55}}
\newcommand{\ceil}[1]{\lceil #1 \rceil}

% MARKUP ------------------------------------------------------------------------------------------

% FORMATTING --------------------------------------------------------------------------------------

\newcommand*{\rout}[1]{\ensuremath{\text{\FuncSty{#1}}}}
%\newcommand*{\mat}[1]{\ensuremath{\boldsymbol{#1}}}
\newcommand*{\mat}[1]{\ensuremath{\mathrm{#1}}}
\renewcommand*{\vec}[1]{\ensuremath{\boldsymbol{#1}}}
\newcommand*{\base}[1]{\ensuremath{\boldsymbol{#1}}}



% GREEK LETTERS -----------------------------------------------------------------------------------
\let\sbphi\phi
\renewcommand*{\phi}{\varphi}
%\renewcommand*{\theta}{\vartheta}
\renewcommand*{\rho}{\varrho}
\newcommand*{\veps}{\varepsilon}
\renewcommand*{\subset}{\subseteq}

%\renewcommand*{\Gamma}{\varGamma}
%\renewcommand*{\Delta}{\varDelta}
%\renewcommand*{\Theta}{\varTheta}
%\renewcommand*{\Lambda}{\varLambda}
%\renewcommand*{\Xi}{\varXi}
%\renewcommand*{\Pi}{\varPi}
%\renewcommand*{\Sigma}{\varSigma}
%\renewcommand*{\Upsilon}{\varUpsilon}
%\renewcommand*{\Phi}{\varPhi}
%\renewcommand*{\Psi}{\varPsi}
%\renewcommand*{\Omega}{\varOmega}


% LATIN -------------------------------------------------------------------------------------------

\newcommand*{\latinabbr}[1]{#1}
%\newcommand*{\latinabbr}[1]{\textit{#1}}
\newcommand*{\ie}{\latinabbr{i.e.}} % id est
\newcommand*{\eg}{\latinabbr{e.g.}} % exemplī grātiā
\newcommand*{\etc}{\latinabbr{etc.}} % et cetera


% COMMON MATHEMATICAL SYMBOLS ---------------------------------------------------------------------

\newcommand*{\defeq}{\ensuremath{\coloneqq}}
\newcommand*{\eqdef}{\ensuremath{\eqqcolon}}

\newcommand*{\dual}{\ensuremath{\ast}}
\renewcommand*{\star}{\ensuremath{\ast}}

\newcommand*{\dd}{\ensuremath{\mathrm{d}}}
\newcommand*{\dx}[1]{\ensuremath{\,\dd{#1}}}
\newcommand*{\dmx}[2]{\ensuremath{\,\dd{#1(#2)}}}

\newcommand*{\grad}{\ensuremath{\nabla}}
\newcommand*{\divg}{\ensuremath{\nabla\cdot}}
%\newcommand*{\gradx}{\ensuremath{\nabla_x}}
%\newcommand*{\divgx}{\ensuremath{\nabla_x\cdot}}
\newcommand*{\laplace}{\ensuremath{\Updelta}}

\newcommand*{\RR}{\ensuremath{\mathbb{R}}}
\newcommand*{\CC}{\ensuremath{\mathbb{C}}}
\newcommand*{\CCo}{\ensuremath{\bar{\mathbb{C}}}}
\newcommand*{\NN}{\ensuremath{\mathbb{N}}}
\newcommand*{\PP}{\ensuremath{\mathbb{P}}}
\newcommand*{\ZZ}{\ensuremath{\mathbb{Z}}}
\newcommand*{\QQ}{\ensuremath{\mathbb{Q}}}
\newcommand*{\KK}{\ensuremath{\mathbb{K}}}
\newcommand*{\POD}{{\text{POD}}}

% left-pointing maps to
\newcommand*{\mapsfrom}{\ensuremath{\leftarrow}}

%{\mathrel{\reflectbox{\ensuremath{\mapsto}}}}
%$\mathrel{\reflectbox{$\mapsto$}}$

% MATH OPERATORS ----------------------------------------------------------------------------------

\DeclareMathOperator{\id}{id}
\DeclareMathOperator{\Id}{Id}
\DeclareMathOperator{\tr}{tr}
\DeclareMathOperator{\conv}{conv}
\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\linspan}{span}
\DeclareMathOperator{\diam}{diam}
\DeclareMathOperator{\ddiv}{div}
\DeclareMathOperator{\spn}{span}
\DeclareMathOperator{\proj}{proj}
\DeclareMathOperator{\diag}{diag}

\newcommand*{\essinf}{\mathop{\mathrm{ess\,inf}}\displaylimits}
\newcommand*{\esssup}{\mathop{\mathrm{ess\,sup}}\displaylimits}

\DeclareMathOperator{\argmin}{argmin}
\DeclareMathOperator{\argmax}{argmax}


% NORMS, INNER PRODUCTS, ETC ----------------------------------------------------------------------

% the first (optional) argument is meant for \big, \Big, \bigg or \Bigg
\newcommand*{\abs}[2][{}]{\ensuremath{#1\left\lvert#2#1\right\rvert}}
\newcommand*{\norm}[2][{}]{\ensuremath{#1\left\Vert#2#1\right\Vert}}
\newcommand*{\dupair}[3][{}]{\ensuremath{#1\langle #2, #3#1\rangle}}
\newcommand*{\scapro}[3][{}]{\ensuremath{#1( #2, #3#1)}}
\newcommand*{\menge}[3][{}]{\ensuremath{#1\{ #2 \,;\: #3#1\}}}
\newcommand*{\inner}[2]{\ensuremath{\left\langle #1, #2 \right\rangle}}
\newcommand*{\hnorm}[1]{\ensuremath{\left\Vert #1 \right\Vert_{H^1}}}
\newcommand*{\tIk}{\ensuremath{\tilde{\mathcal{I}}_k}}



\newcommand*{\inpol}{\ensuremath{\mathcal{I}_{\mathbf{p^{(\ell)}}}}}
\newcommand*{\bfeta}{\ensuremath{\mathbf{\eta}}}
\newcommand*{\bfu}{\ensuremath{\mathbf{u}}}
\newcommand*{\bfx}{\ensuremath{\mathbf{x}}}
\newcommand*{\bfz}{\ensuremath{\mathbf{z}}}
\newcommand*{\bfy}{\ensuremath{\mathbf{y}}}
\newcommand*{\bfv}{\ensuremath{\mathbf{v}}}
\newcommand*{\bfw}{\ensuremath{\mathbf{w}}}
\newcommand*{\bfk}{\ensuremath{\mathbf{k}}}
\newcommand*{\bff}{\ensuremath{\mathbf{f}}}
\newcommand*{\bfb}{\ensuremath{\mathbf{b}}}
\newcommand*{\bfa}{\ensuremath{\mathbf{a}}}
\newcommand*{\bfc}{\ensuremath{\mathbf{c}}}
\newcommand*{\bfd}{\ensuremath{\mathbf{d}}}
\newcommand*{\bfg}{\ensuremath{\mathbf{g}}}
\newcommand*{\bfr}{\ensuremath{\mathbf{r}}}
\newcommand*{\bfe}{\ensuremath{\mathbf{e}}}
\newcommand*{\bfh}{\ensuremath{\mathbf{h}}}
\newcommand*{\bfkappa}{{\ensuremath{\boldsymbol{\kappa}}}}
\newcommand*{\bfpi}{{\ensuremath{\boldsymbol{\pi}}}}
\newcommand*{\bfsbphi}{{\ensuremath{\boldsymbol{\sbphi}}}}
\newcommand*{\nn}{\ensuremath{\text{NN}}}
\newcommand*{\kp}{\ensuremath{\mathcal{K}_{\mathbf{p}^{(\ell)}}}}
\DeclareMathOperator{\E}{\mathbb{E}}

% GENERAL FUNCTION SPACES -------------------------------------------------------------------------

% just the function space
\newcommand*{\Lp}[1][2]{\ensuremath{L^{#1}}}
\newcommand*{\lp}[1][2]{\ensuremath{\ell^{#1}}}
\newcommand*{\Hs}[1][1]{\ensuremath{H^{#1}}}
\newcommand*{\Hso}[1][1]{\ensuremath{H^{#1}_0}}
\newcommand*{\Cont}[1][{}]{\ensuremath{C^{#1}}}
\newcommand*{\Lop}{\ensuremath{\mathcal{L}}}
\newcommand*{\Wsp}[2]{\ensuremath{W^{#1,#2}}}

% function space with a domain
\newcommand*{\Lps}[2][2]{\ensuremath{\Lp[#1](#2)}}
\newcommand*{\lps}[2][2]{\ensuremath{\lp[#1](#2)}}
\newcommand*{\Lpms}[3][2]{\ensuremath{\Lp[#1]_{#2}(#3)}}
\newcommand*{\Hss}[2][1]{\ensuremath{\Hs[#1](#2)}}
\newcommand*{\Hsos}[2][1]{\ensuremath{\Hso[#1](#2)}}
\newcommand*{\Conts}[2][{}]{\ensuremath{\Cont[#1](#2)}}
\newcommand*{\Wsps}[3]{\ensuremath{\Wsp{#1}{#2}(#3)}}

% bochner spaces
\newcommand*{\Lpsv}[3][2]{\ensuremath{\Lp[#1](#2;#3)}}
\newcommand*{\lpsv}[3][2]{\ensuremath{\lp[#1](#2;#3)}}
\newcommand*{\Lpmsv}[4][2]{\ensuremath{\Lp[#1]_{#2}(#3;#4)}}
\newcommand*{\Hssv}[3][1]{\ensuremath{\Hs[#1](#2;#3)}}
\newcommand*{\Contsv}[3][{}]{\ensuremath{\Cont[#1](#2;#3)}}


% DOMAINS -----------------------------------------------------------------------------------------

% spatial domain
\newcommand*{\dom}{\ensuremath{D}}
\newcommand*{\dombd}{\ensuremath{\partial\dom}}
\newcommand*{\dombdD}{\ensuremath{\partial\dom_D}}
\newcommand*{\dombdN}{\ensuremath{\partial\dom_N}}

% parameter domain
\newcommand{\pdom}{\ensuremath{\Gamma}}
\newcommand{\pmsr}{\ensuremath{\pi}}


% INDEX SETS --------------------------------------------------------------------------------------

% all tensor product polynomials
\newcommand*{\indx}{\ensuremath{\mathcal{F}}}

% active tensor product polynomials
\newcommand*{\ipol}{\ensuremath{\Lambda}}

% some subset
\newcommand*{\subipol}{\ensuremath{\Delta}}

% exterior boundary of active basis elements
\newcommand*{\ebd}{\ensuremath{\partial}}

% exterior boundary of active basis elements within active dimensions
\newcommand*{\aebd}{\ensuremath{\ebd^\circ\!}}

% marked multiindices
\newcommand*{\mimarked}{\ensuremath{\Delta}}

% marked dimensions
\newcommand*{\dimmarked}{\ensuremath{\Sigma}}

% kronecker sequence
\newcommand*{\kron}{\ensuremath{\epsilon}}


% OPERATORS AND SESQUILINEAR FORMS ----------------------------------------------------------------

% coefficient in elliptic differential operator
\newcommand*{\ac}{\ensuremath{a}}
\newcommand*{\aco}{\ensuremath{\bar{a}}}
\newcommand*{\acm}{\ensuremath{a}}
\newcommand*{\acmin}{\ensuremath{a_{\mathrm{min}}}}
\newcommand*{\acmax}{\ensuremath{a_{\mathrm{max}}}}
\newcommand*{\nsbnd}{\ensuremath{\gamma}}
\newcommand*{\nuc}{\ensuremath{\nu}}
\newcommand*{\nuco}{\ensuremath{\bar{\nu}}}
\newcommand*{\nucm}{\ensuremath{\nu}}
\newcommand*{\nucmin}{\ensuremath{\nu_{\mathrm{min}}}}
\newcommand*{\nucmax}{\ensuremath{\nu_{\mathrm{max}}}}
\newcommand*{\sigmao}{\ensuremath{\bar{\sigma}}}
\newcommand*{\sigmam}{\ensuremath{\sigma}}
\newcommand*{\sigmamin}{\ensuremath{\sigma_{\mathrm{min}}}}
\newcommand*{\sigmamax}{\ensuremath{\sigma_{\mathrm{max}}}}
\newcommand*{\Eo}{\ensuremath{\bar{E}}}
\newcommand*{\Em}{\ensuremath{E}}
\newcommand*{\Emin}{\ensuremath{E_{\mathrm{min}}}}
\newcommand*{\Emax}{\ensuremath{E_{\mathrm{max}}}}
\newcommand*{\mcC}{\ensuremath{\mathcal{C}}}
\newcommand*{\lo}{\ensuremath{\bar{\lambda}}}
\newcommand*{\lm}{\ensuremath{\lambda}}
\newcommand*{\lmin}{\ensuremath{\lambda_{\mathrm{min}}}}
\newcommand*{\lEmax}{\ensuremath{\lambda_{\mathrm{max}}}}


% elliptic sesquilinear forms and operators
\newcommand*{\Ay}{\ensuremath{A}}
\newcommand*{\As}{\ensuremath{\mathcal{A}}}
\newcommand*{\Ao}{\ensuremath{\bar{A}}}
\newcommand*{\Am}{\ensuremath{A}}
\newcommand*{\Aos}{\ensuremath{\bar{\mathcal{A}}}}

% discrete operators
\newcommand*{\Ac}{\ensuremath{\mat{A}}}
\newcommand*{\Aoc}{\ensuremath{\mat{\bar{A}}}}

% residual
\newcommand*{\Resi}{\ensuremath{\mathcal{R}}}


% multiplication by y_m
\newcommand*{\multm}{\ensuremath{K}}
\newcommand*{\multmat}{\ensuremath{\mat{K}}}


% SPACES IN PARAMETRIC PROBLEM --------------------------------------------------------------------

% spaces in x
\newcommand*{\varspc}{\ensuremath{V}}

% abstract finite element space
\newcommand*{\fespc}{\ensuremath{V}}
\newcommand*{\galspc}{\ensuremath{\mathcal{V}}}
\newcommand*{\cospc}{\ensuremath{\boldsymbol{V}}}

% approximation space
\newcommand*{\apspc}{\ensuremath{\mathbb{A}}}


% FE MESHES --------------------------------------------------------------------------------------------------------

% elements
\newcommand*{\cell}{\ensuremath{T}}
\newcommand*{\face}{\ensuremath{S}}
\newcommand*{\cellbd}{\ensuremath{\partial\cell}}
\newcommand*{\cellneigh}{\ensuremath{\tilde{\omega}}}
\newcommand*{\cellnei}{\ensuremath{\omega}}

% mesh
\newcommand*{\mesh}{\ensuremath{\mathcal{T}}}
\newcommand*{\faces}{\ensuremath{\mathcal{S}}}
%\newcommand*{\initmesh}{\ensuremath{\mathcal{\mathring{T}}}}
\newcommand*{\initmesh}{\ensuremath{\mathcal{{T_{\mathrm{init}}}}}}
\newcommand*{\admismesh}{\ensuremath{\mathbb{T}}}
\newcommand*{\submesh}{\ensuremath{\mathcal{M}}}
\newcommand*{\marked}{\ensuremath{\mathcal{M}}}

% clement interpolant
\newcommand*{\clint}{\ensuremath{\mathcal{I}}}

% normal jump
\newcommand*{\jump}[1]{\ensuremath{ [\![ #1 ]\!] }}

% oscillation
\DeclareMathOperator{\osc}{osc}

% partial order on meshes
\newcommand*{\coarser}{\ensuremath{\preceq}}
\newcommand*{\overlay}{\ensuremath{\oplus}}
\newcommand*{\bigoverlay}{\ensuremath{\bigoplus}}

% stuff for paper
\newcommand*{\Ul}{\ensuremath{\mathcal{U}_\ell}}

\newcommand*{\net}{\mathcal{N}\hspace*{-1pt}\mathcal{N}}
